Color superconductivity from the chiral quark-meson model

We study the two-flavor color superconductivity of low-temperature quark matter in the vicinity of chiral phase transition in the quark-meson model where the interactions between quarks are generated by pion and sigma exchanges. Starting from the Nambu-Gor'kov propagator in real-time formulation we obtain finite temperature (real axis) Eliashberg-type equations for the quark self-energies (gap functions) in terms of the in-medium spectral function of mesons. Exact numerical solutions of the coupled nonlinear integral equations for the real and imaginary parts of the gap function are obtained in the zero temperature limit using a model input spectral function. We find that these components of the gap display a complicated structure with the real part being strongly suppressed above $2\Delta_0$, where $\Delta_0$ is its on-shell value. We find $\Delta_0\simeq 40$ MeV close to the chiral phase transition.

==> aas.tex <==
% -------------------------- AASTEX ACRONYMS -------------
\def\aapr{Astronomy and Astrophysics Reviews}
\def\aj{AJ}%
          % Astronomical Journal 
\def\actaa{Acta Astron.}%
          % Acta Astronomica 
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys 
\def\apj{ApJ \ }%
          % Astrophysical Journal 
\def\apjl{ApJ \ }%
          % Astrophysical Journal, Letters 
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement 
\def\ao{Appl. Opt.}%
          % Applied Optics 
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science 
\def\aap{A\&A}%
          % Astronomy and Astrophysics 
\def\aapr{A\&A Rev.}%
          % Astronomy and Astrophysics Reviews 
\def\aaps{A\&A}%
          % Astronomy and Astrophysics, Supplement 
\def\azh{AZh}%
          % Astronomicheskii Zhurnal 
\def\baas{BAAS}%
          % Bulletin of the AAS 
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics 
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics 
\def\icarus{Icarus}%
          % Icarus 
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics 
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada 
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS 
\def\memras{MmRAS}%
          % Memoirs of the RAS 
\def\na{New A}%
          % New Astronomy 
\def\nar{New A Rev.}%
          % New Astronomy Review 
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia 
\def\pra{Phys. Rev. A\ }%
          % Physical Review A: General Physics 
\def\prb{Phys. Rev. B \ }%
          % Physical Review B: Solid State 
\def\prc{Phys. Rev. C\ }%
          % Physical Review C 
\def\prd{Phys. Rev. D \ }%
          % Physical Review D 
\def\pre{Phys. Rev. E \ }%
          % Physical Review E 
\def\prl{Phys. Rev. Lett. \ }%
          % Physical Review Letters 
\def\pasp{PASP}%
          % Publications of the ASP 
\def\pasj{PASJ}%
          % Publications of the ASJ 
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS 
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica 
\def\skytel{S\&T}%
          % Sky and Telescope 
\def\solphys{Sol. Phys.}%
          % Solar Physics 
\def\sovast{Soviet Ast.}%
          % Soviet Astronomy 
\def\ssr{Space Sci. Rev.}%
          % Space Science Reviews 
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik 
\def\nat{Nature}%
          % Nature 
\def\iaucirc{IAU Circ.}%
          % IAU Cirulars 
\def\aplett{Astrophys. Lett.}%
          % Astrophysics Letters 
\def\apspr{Astrophys. Space Phys. Res.}%
          % Astrophysics Space Physics Research 
\def\bain{Bull. Astron. Inst. Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands 
\def\fcp{Fund. Cosmic Phys.}%
          % Fundamental Cosmic Physics 
\def\gca{Geochim. Cosmochim. Acta}%
          % Geochimica Cosmochimica Acta 
\def\grl{Geophys. Res. Lett.}%
          % Geophysics Research Letters 
\def\jcp{J. Chem. Phys.}%
          % Journal of Chemical Physics 
\def\jgr{J. Geophys. Res.}%
          % Journal of Geophysics Research 
\def\jqsrt{J. Quant. Spec. Radiat. Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\def\memsai{Mem. Soc. Astron. Italiana}%
          % Mem. Societa Astronomica Italiana 
\def\nphysa{Nucl. Phys. A}%
          % Nuclear Physics A 
\def\physrep{Phys. Rep. \ }%
          % Physics Reports 
\def\physscr{Phys. Scr}%
          % Physica Scripta 
\def\planss{Planet. Space Sci.}%
          % Planetary Space Science 
\def\procspie{Proc. SPIE}%
          % Proceedings of the SPIE 

